Object-aware Video-language Pre-training for Retrieval

Recently, by introducing large-scale dataset and strong transformer network, video-language pre-training has shown great success especially for retrieval. Yet, existing video-language transformer models do not explicitly fine-grained semantic align. In this work, we present Object-aware Transformers, an object-centric approach that extends video-language transformer to incorporate object representations. The key idea is to leverage the bounding boxes and object tags to guide the training process. We evaluate our model on three standard sub-tasks of video-text matching on four widely used benchmarks. We also provide deep analysis and detailed ablation about the proposed method. We show clear improvement in performance across all tasks and datasets considered, demonstrating the value of a model that incorporates object representations into a video-language architecture. The code will be released at \url{https://github.com/FingerRec/OA-Transformer}.

==> figures/4_Mask_visualize.tex <==
\begin{figure}
  \centering
   \includegraphics[width=.7\linewidth]{figures/src/mask_visualization.pdf}

   \caption{
   \textbf{ The most informative region are preserved with object-guided masking operation with the vary of time.}
   We first get the patches that include the conspicuous object according to predicted high-confidential prediction.
   Then these patches are preserved while the others are masked.
   The number means the temporal index.
   }
   \label{fig:4_mask_vis}
\end{figure}



==> tables/ref_table.tex <==
\begin{table}[t]
\begin{tabular}{l|rrr|rr|rr}
& \multicolumn{3}{c|}{\scriptsize IN1K}
& \multicolumn{2}{c|}{\scriptsize COCO}
& \multicolumn{2}{c}{\scriptsize ADE20K} \\
& \scriptsize ViT-B & \scriptsize ViT-L & \scriptsize ViT-H
& \scriptsize ViT-B & \scriptsize ViT-L
& \scriptsize ViT-B & \scriptsize ViT-L \\
\shline
pixel (w/o norm) & 83.3 & 85.1 & 86.2 & 49.5 & 52.8 & 48.0 & 51.8 \\
pixel (w/ norm) & 83.6 & 85.9 & 86.9 & 50.3 & 53.3 & 48.1 & 53.6 \\
\hline
dVAE token & 83.6 & 85.7 & 86.9 & 50.3 & 53.2 & 48.1 & 53.4 \\
$\triangle$ & 0.0 & -0.2 & 0.0 & 0.0 & -0.1 & 0.0 & -0.2
\end{tabular}
\vspace{-.7em}
\caption{\textbf{Pixels \vs tokens} as the MAE reconstruction target. $\triangle$ is the difference between using dVAE tokens and using normalized pixels. The difference is statistically insignificant.}
\label{tab:pixel_vs_token}
\end{table}
